Scalable Sensitivity and Uncertainty Analysis for Causal-Effect Estimates of Continuous-Valued Interventions

Estimating the effects of continuous-valued interventions from observational data is a critically important task for climate science, healthcare, and economics. Recent work focuses on designing neural network architectures and regularization functions to allow for scalable estimation of average and individual-level dose-response curves from high-dimensional, large-sample data. Such methodologies assume ignorability (observation of all confounding variables) and positivity (observation of all treatment levels for every covariate value describing a set of units), assumptions problematic in the continuous treatment regime. Scalable sensitivity and uncertainty analyses to understand the ignorance induced in causal estimates when these assumptions are relaxed are less studied. Here, we develop a continuous treatment-effect marginal sensitivity model (CMSM) and derive bounds that agree with the observed data and a researcher-defined level of hidden confounding. We introduce a scalable algorithm and uncertainty-aware deep models to derive and estimate these bounds for high-dimensional, large-sample observational data. We work in concert with climate scientists interested in the climatological impacts of human emissions on cloud properties using satellite observations from the past 15 years. This problem is known to be complicated by many unobserved confounders.

==> sections/methods/bound_estimator_old.tex <==
\subsection{Continuous Treatment Effect Interval Estimator}
\label{sec:estimator}
Following \cite{jesson2021quantifying}, we develop a parametric estimator of the bounds in \Cref{def:CAPO_bounds,def:APO_bounds}. 
The parametric estimator is based off of the doubly-robust formulation of \Cref{eq:mu_w}:
\begin{equation}
    \begin{split}
        \mu&(w(\y); \x, \tf) \\
        &= \mut(\x, \tf) + \frac{\int_\Ycal r(\y; \tf, \x) w(\y; \tf, \x)p(\y \mid \tf, \x)d\y}{\int_\Ycal w(\y; \tf, \x)p(\y \mid \tf, \x)d\y},
    \end{split}
\end{equation}
where $r(\y; \tf, \x) = y - \mut(\x, \tf)$.

By analogy to Lemma 3 in \cite{jesson2021quantifying}, the lower bound in \Cref{def:CAPO_bounds} is given by,
\begin{equation}
    \underline{\mu}(\x, \tf; \Lambda) = \inf_{u \in \Uni} \{ \kappa(\x, \tf; \Lambda, u) \},
\end{equation}
where $\Uni = \{ u: \Ycal \to [0, 1] \: \textrm{s.t}.\: u(\y) \: \textrm{is non-increasing} \}$,
\begin{equation*}
    \begin{split}
        \kappa(\x, &\tf; \Lambda, u) = \\
        &\mut(\x, \tf) + \frac{\int u(\y) r(\y; \tf, \x) p(\y | \tf, \x)d\y}{\alphap\left(\x; \Lambda, p(\tf \mid \x)\right) + \int u(\y)p(\y | \tf, \x)d\y},
    \end{split}
    \label{eq:kappa}
\end{equation*}
and 
\begin{equation*}
    \alphap(\x; \Lambda, p(\tf \mid, \x)) = \frac{\alpha(p(\tf \mid \x), \Lambda)}{\beta(p(\tf \mid \x), \Lambda) - \alpha(p(\tf \mid \x), \Lambda)}.
    \label{eq:gamma}
\end{equation*}
Similarly, the upper bound in \Cref{def:CAPO_bounds} is given by,
\begin{equation}
        \overline{\mu}(\x, \tf; \Lambda) = \sup_{u \in \Und} \{ \kappa(\x, \tf; \Lambda, u) \},
\end{equation}
where $\Und = \{ u: \Ycal \to [0, 1] \: \textrm{s.t}.\: u(\y) \: \textrm{is non-decreasing} \}$.

Given this formulation, the bounds on the expected potential outcome, $\mu(\x, \tf)$, are now completely defined in terms of identifiable quantities: namely, the nominal propensity density for treatment, $p(\tf \mid \x)$; the conditional density of the outcome given the assigned treatment and measured covariates, $p(\y \mid \tf, \x)$; and the conditional expected outcome $\mut(\x, \tf)$. 
Thus, we define density estimators $\pp(\tf \mid \x)$, $\pp(\y \mid \tf, \x)$, and estimator $\mup(\x, \tf)$ parameterized by instances $\params$ of the random variable $\Params$.
% The bounds on the expected potential outcome, $\mu(\x, \tf)$, are now completely defined in terms of identifiable quantities: namely, the conditional density of the outcome given the assigned treatment and measured covariates, $p(\y \mid \tf, \x)$; and the conditional expected outcome $\mut(\x, \tf)$. 
% Thus, we define density estimators $\pp(\tf \mid \x)$, $\pp(\y \mid \tf, \x)$, and estimator $\mup(\x, \tf)$ parameterized by instances $\params$ of the random variable $\Params$.

In this work we will model both densities as Gaussian mixtures, noting that with a sufficient number of components they can model any continuous distribution \cite{titterington1985statistical}. Thus,
\begin{equation*}
    \pp(\tf \mid \x) = \sum_{j=1}^{n_{\tf}} \pip^{j}(\x) \mathcal{N}\left(\tf \mid \mup^{j}(\x), \Sigmap^{j}(\x)\right),
\end{equation*}
\begin{equation*}
    \pp(\y \mid \tf, \x) = \sum_{j=1}^{n_{\y}} \pip^{j}(\x, \tf) \mathcal{N}\left(\y \mid \mup^{j}(\x, \tf), \sigmap^{2j}(\x, \tf)\right),
\end{equation*}
and $\mup(\x, \tf) = \sum_{j=1}^{n_{\y}} \pip^{j}(\x, \tf)\mup^{j}(\x, \tf)$ \cite{bishop1994mixture}.

The parametric bound estimators of the CAPO function are then given by,
\begin{equation*}
    \underline{\mu}_{\params}(\x, \tf; \Lambda) = \inf_{u \in \Uni} \left\{ \kappap(\x, \tf; \Lambda, u) \right\},
\end{equation*}
and
\begin{equation*}
    \overline{\mu}_{\params}(\x, \tf; \Lambda) = \sup_{u \in \Und} \{ \kappap(\x, \tf; \Lambda, u) \},
\end{equation*}
where
\begin{equation}
    \begin{split}
        \kappap&(\x, \tf; \Lambda, u) = \\
        &\mup + 
        \frac{\int u(\y) r_{\params}(\y; \tf, \x) \pp(\y | \tf, \x)d\y}
        {\alphap\left(\x; \Lambda, \pp(\tf \mid \x)\right) + \int u(\y)\pp(\y | \tf, \x)d\y},
    \end{split}
    \label{eq:kappap}
\end{equation}
where $\mup=\mup(\x, \tf)$.
Finally, the parametric bound estimators for the APO (dose-response) function are given by,
\begin{equation}
    \underline{\mu}_{\params}(\tf; \Lambda) = \inf_{u \in \Uni}  \E[\kappap(\X, \tf; \Lambda, u)],
\end{equation}
and
\begin{equation}
    \overline{\mu}_{\params}(\tf; \Lambda) = \sup_{u \in \Und} \E[\kappap(\X, \tf; \Lambda, u)].
\end{equation}

==> sections/methods/interval_estimator_0.tex <==
\subsection{Solving for $w$}
\label{sec:algorithm}
We are interested in a scalable algorithm to compute the intervals on the CAPO function and the APO function.
To calculate the bounds on the APO (dose-response) function, the bounds on  the CAPO function must be computed at each datapoint.
The bounds on the CAPO function can be calculated independently for each instance $\X=\x$; however, the bounds on the APO are taken with respect to an expectation over $\X$, so a batched algorithm can facilitate scalability.
Furthermore, the need for scalability is compounded by the need to evaluate the intervals at multiple values of the continuous treatment variable $\tf \in \Tcal$, which could be arbitrarily many.
We consider three different solutions below: a parallel \emph{line search} approach; a batched \emph{grid search} approach; and a batched \emph{gradient descent} approach.
\subsubsection{Selecting the appropriate class of $u$ functions}
Step function
\begin{equation*}
    H(\y) \coloneqq 
    \begin{dcases*}
        1, \y > \ystar \\
        0, \y \leq \ystar
    \end{dcases*}
\end{equation*}
\begin{equation*}
    \Und_H = \left\{ H(\y - \ystar): \ystar \in \Ycal \right\}
\end{equation*}
\begin{equation*}
    \Uni_H = \left\{ H(\ystar - \y): \ystar \in \Ycal \right\}
\end{equation*}

Differentiable sigmoid function
\begin{equation*}
    S(y) \coloneqq \left( 1 + \exp{(-y)} \right)^{-1}
\end{equation*}
\begin{equation*}
    \Und_S = \left\{ S\left(\frac{\y - \ystar}{s}\right): \ystar \in \Ycal \right\}
\end{equation*}
\begin{equation*}
    \Uni_S = \left\{ S\left(\frac{\ystar - \y}{s}\right): \ystar \in \Ycal \right\}
\end{equation*}

\subsubsection{Approximating the integrals in $\kappap(\x, \tf; \Lambda, u)$ using Gauss-Hermite quadrature}
Gauss-Hermite quadrature is a numerical method to approximate indefinite integrals of the following form: $\int_{-\infty}^{\infty}\exp{(-\y^2)f(\y)d\y}$.
In this case,
\begin{equation*}
    \int_{-\infty}^{\infty}\exp{(-\y^2)f(\y)d\y} \approx \sum_{i=1}^{m}w_i f(\y),
\end{equation*}
where $m$ is the number of samples drawn. The $\y_i$ are the roots of the physicists Hermite polynomial $H^*_{m}(\y)(i=1, 2, \dots, m)$ and the weights are given by
\begin{equation*}
    w_i = \frac{2^{m-1}m!\sqrt{\pi}}{m^2[H^*_{m-1}(\y_k)]^2}
\end{equation*}
This method can be used to calculate the expectation of a function, $h(y)$, with respect to Gaussian distributed $\y \sim \mathcal{N}(\mu, \sigma^2)$ through a change of variables, such that,
\begin{equation*}
    \begin{split}
        \E_{\mathcal{N}(\mu, \sigma^2)}[h(\y)] &= \int_{-\infty}^{\infty} \frac{1}{\sqrt{\pi}}\exp{\left( -\y^2 \right)} h\left( \sqrt{2}\sigma \y + \mu \right) d\y   \\
        &\approx \frac{1}{\sqrt{\pi}} \sum_{i=1}^{m}w_i h\left( \sqrt{2}\sigma \y + \mu \right).
    \end{split}
\end{equation*}
We would like to approximate the expectation of a function, either $h(\y) = u(\y) r_{\params}(\y; \tf, \x)$ or $h(\y) = u(\y)$, with respect to our density estimator $\pp(\y | \tf, \x)$, which is a Gaussian mixture. Thus,
\begin{equation*}
    \begin{split}
        \E_{\pp(\y | \tf, \x)}&[h(\y)] = \\
        & \frac{1}{\sqrt{\pi}} \sum_{j=1}^{n_{\tf}} \pip^{j} \int_{-\infty}^{\infty} \exp{\left( -\y^2 \right)} h\left( \sqrt{2}\sigmap^{2j} \y + \mup^{j} \right) d\y
    \end{split}
\end{equation*}
where, $\pip^{j}=\pip^{j}(\x)$, $\mup^{j}=\mup^{j}(\x, \tf)$, and $\sigmap^{2j}=\sigmap^{2j}(\x, \tf)$.
\begin{definition}
\label{def:integral-estimator}
{\normalfont Gauss-Hermite quadrature integral estimator}
    \begin{equation*}
        I(h(\y)) \coloneqq \frac{1}{\sqrt{\pi}} \sum_{j=1}^{n_{\tf}} \pip^{j} \sum_{i=1}^{m} w_i h\left( \sqrt{2}\sigmap^{2j}(\x, \tf) \y + \mup^{j} \right)
    \end{equation*}
\end{definition}
We can now plug this into \Cref{eq:kappap} to define the following estimator:
\begin{equation*}
    \widehat{\kappa}_{\params}(\x, \tf; \Lambda, u) \coloneqq \mup + \frac{I(u(\y) r_{\params}(\y; \tf, \x))}{\alphap\left(\x; \Lambda, \pp(\tf \mid \x)\right) + I(u(\y))}.
\end{equation*}

\subsubsection{Discrete search approaches}
Let $\widehat{\Ycal}=\{\y_i \in \Ycal\}_{i=1}^{k}$ be a set of $k$ values of $\y$, then
\begin{equation*}
    \begin{split}
         \underline{\mu}_{\params}^{H}(\x, \tf) &= \min_{\ystar} \left\{ \widehat{\kappa}_{\params}(\x, \tf; \Lambda, H(\ystar - \y)): \ystar \in \widehat{\Ycal} \right\}, \\
         \overline{\mu}_{\params}^{H}(\x, \tf) &= \max_{\ystar} \left\{ \widehat{\kappa}_{\params}(\x, \tf; \Lambda, H(\y - \ystar)): \ystar \in \widehat{\Ycal} \right\}.
    \end{split}
\end{equation*}

\begin{algorithm}
    \caption{Grid Search Interval Optimizer}
    \label{alg:grid-search}
    \begin{algorithmic}[1]
        \Require{$\x^{*}$ is an instance of $\X$, $\tf^{*}$ is a treatment level to evaluate, $\Lambda$ is a belief in the amount of hidden confounding, $\params$ are optimized model parameters, $\widehat{\Ycal}$ is a set of unique values $\y \in \Ycal$.}
        \Function{GridSearch}{$\x^{*}$, $\tf^{*}$, $\Lambda$, $\params$, $\widehat{\Ycal}$}
            \State $\overline{\mu} \gets -\infty$
            \State $\underline{\mu} \gets \infty$
            \For{$\ystar \in \widehat{\Ycal}$}
                \State $\overline{\kappa} \gets \widehat{\kappa}_{\params}(\x^{*}, \tf^{*}; \Lambda, H(\y - \ystar))$
                \State $\underline{\kappa} \gets \widehat{\kappa}_{\params}(\x^{*}, \tf^{*}; \Lambda, H(\ystar-\y))$
                \If{$\overline{\kappa} > \overline{\mu}$}
                    \State $\overline{\mu}\gets \overline{\kappa}$
                \EndIf
                \If{$\underline{\kappa} < \underline{\mu}$}
                    \State $\underline{\mu} \gets \underline{\kappa}$
                \EndIf
            \EndFor
            \State \Return $\underline{\mu}, \overline{\mu}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{Line Search Interval Optimizer}
    \label{alg:line-search}
    \begin{algorithmic}[1]
        \Require{$\x^{*}$ is an instance of $\X$, $\tf^{*}$ is a treatment level to evaluate, $\Lambda$ is a belief in the amount of hidden confounding, $\params$ are optimized model parameters, $\widehat{\Ycal}$ is a set of unique values $\y \in \Ycal$ \emph{sorted in ascending order}.}
        \Function{LineSearch}{$\x^{*}$, $\tf^{*}$, $\Lambda$, $\params$, $\widehat{\Ycal}$}
            \State $\overline{\mu} \gets -\infty$, $\overline{\kappa} \gets \infty$
            \State $\underline{\mu} \gets \infty$, $\underline{\kappa} \gets -\infty$
            \State $\underline{\delta} \gets $ True, $\overline{\delta} \gets $ True
            \While{$\underline{\delta}$}
                \State $\ystar \gets \textsc{Pop}(\widehat{\Ycal}_c)$ \Comment{$\widehat{\Ycal}_c$ a copy of $\widehat{\Ycal}$}
                \State $\underline{\kappa} \gets \widehat{\kappa}_{\params}(\x, \tf; \Lambda, H(\ystar-\y))$
                \If{$\underline{\kappa} < \underline{\mu}$}
                    \State $\underline{\mu} \gets \underline{\kappa}$
                \Else 
                    \State $\underline{\delta} \gets $ False
                \EndIf
            \EndWhile
            \While{$\overline{\delta}$}
                \State $\ystar \gets \textsc{Pop}(\widehat{\Ycal}_c)$ \Comment{$\widehat{\Ycal}_c$ a copy of $\widehat{\Ycal}$}
                \State $\overline{\kappa} \gets \widehat{\kappa}_{\params}(\x, \tf; \Lambda, H(\y - \ystar))$
                \If{$\overline{\kappa} > \overline{\mu}$}
                    \State $\overline{\mu} \gets \overline{\kappa}$
                \Else 
                    \State $\overline{\delta} \gets $ False
                \EndIf
            \EndWhile
            \State \Return $\underline{\mu}, \overline{\mu}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}

\subsubsection{Gradient descent approach}
Define $\bm{\omega} \coloneqq \begin{bmatrix} \ystar \\ s \end{bmatrix}$, $\textsc{Softplus}(s) \coloneqq \log{(1 + \exp{(s)})}$, $\underline{S}_{\bm{\omega}}(\y) \coloneqq S\left(\frac{\ystar-\y}{\textsc{Softplus}(s) + \zeta}\right)$, and $\overline{S}_{\bm{\omega}}(\y) \coloneqq S\left(\frac{\y-\ystar}{\textsc{Softplus}(s) + \zeta}\right)$, where $\zeta$ is a small positive constant.
Then the gradient descent approach seeks to solve the following optimization problems:
\begin{equation*}
    \begin{split}
        \underline{\mu}_{\params}^{S}(\x, \tf) &= \min_{\bm{\omega}} \widehat{\kappa}_{\params}\left(\x, \tf; \Lambda, \underline{S}_{\bm{\omega}}(\y) \right), \\
        \overline{\mu}_{\params}^{S}(\x, \tf) &= \min_{\bm{\omega}} -\widehat{\kappa}_{\params}\left(\x, \tf; \Lambda, \overline{S}_{\bm{\omega}}(\y) \right).
    \end{split}
\end{equation*}

\begin{algorithm}
    \caption{Gradient Descent Interval Optimizer}
    \label{alg:gradient-descent}
    \begin{algorithmic}[1]
        \Require{$\x^{*}$ is an instance of $\X$, $\tf^{*}$ is a treatment level to evaluate, $\Lambda$ is a belief in the amount of hidden confounding, $\params$ are optimized model parameters.}
        \Function{GradientDescent}{$\x^{*}$, $\tf^{*}$, $\Lambda$, $\params$, $\epsilon$}
            \State $\bm{\omega} \coloneqq \begin{bmatrix} \ystar \\ s \end{bmatrix}$
            \State $\overline{S}_{\bm{\omega}}(\y) \coloneqq S\left(\frac{\y-\ystar}{\textsc{Softplus}(s) + \zeta}\right)$
            \State $\underline{S}_{\bm{\omega}}(\y) \coloneqq S\left(\frac{\ystar-\y}{\textsc{Softplus}(s) + \zeta}\right)$
            \State $i \gets 0$, $\ystar_i \sim \mathcal{N}(0, 1)$, $s_i \gets 0.0$, $\delta \gets \inf$
            \While{$\delta > \epsilon$}
                \State $\underline{\mu} \gets \widehat{\kappa}_{\params}\left(\x, \tf; \Lambda, \underline{S}_{\bm{\omega}_i}(\y)\right)$
                \State $\bm{\omega}_{i+1} = \bm{\omega}_{i} - \eta \nabla_{\bm{\omega}} \underline{\mu}$ 
                \State $\delta = \left\lVert{\bm{\omega}_{i+1} - \bm{\omega}_{i}}\right\rVert$
                \State $i \gets i + 1$
            \EndWhile
            \State $i \gets 0$, $\ystar_i \sim \mathcal{N}(0, 1)$, $s_i \gets 0.0$, $\delta \gets \inf$
            \While{$\delta > \epsilon$}
                \State $\overline{\mu} \gets \widehat{\kappa}_{\params}\left(\x, \tf; \Lambda, \overline{S}_{\bm{\omega}_i}(\y)\right)$
                \State $\bm{\omega}_{i+1} = \bm{\omega}_{i} + \eta \nabla_{\bm{\omega}} \overline{\mu}$ 
                \State $\delta = \left\lVert{\bm{\omega}_{i+1} - \bm{\omega}_{i}}\right\rVert$
                \State $i \gets i + 1$
            \EndWhile
            \State \Return $\underline{\mu}, \overline{\mu}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}

\subsubsection{APO (dose-response) function interval estimator}
The bounds for the APO function interval estimator given observational data $\D$ and the CMSM parameterized by $\Lambda$ are given by,
\begin{equation*}
    \begin{split}
        \underline{\mu}_{\params}^{(\cdot)}(\tf) &\coloneqq \frac{1}{n}\sum_{i=1}^{n_{\D}} \underline{\mu}_{\params}^{(\cdot)}(\x_i, \tf), \\
        \overline{\mu}_{\params}^{(\cdot)}(\tf) &\coloneqq \frac{1}{n}\sum_{i=1}^{n_{\D}} \overline{\mu}_{\params}^{(\cdot)}(\x_i, \tf),
    \end{split}
\end{equation*}
where $(\cdot)$ can either be the step function $H$ or the sigmoid function $S$ depending on the optimization proceedure.

==> sections/methods/uncertainty.tex <==
\subsection{Uncertainty about the Continuous Treatment Effect Interval}
\label{sec:uncertainty}
% \subsubsection{Frequentist interpretation}
Following \cite{zhao2019sensitivity, dorn2021sharp, chernozhukov2021omitted}, we construct $(1 - \alpha)$ confidence intervals for the upper and lower bounds under the CMSM using the percentile bootstrap estimator.
Let $P_{\D}$ be the empirical distribution of the observed data sample, $\D=\{\x_i, \tf_i, \y_i\}_{i=1}^n = \{\mathbf{S}_i\}_{i=1}^n$.
Let $\widehat{P}_{\D} = \{\widehat{\D}_j\}_{k=1}^{n_b}$ be the bootstrap distribution over $n_b$ datasets, $\widehat{\D}_k=\{\widehat{\mathbf{S}}_i\}_{i=1}^n$, sampled with replacement from the empirical distribution, $P_{\D}$.
Let $Q_{\alpha}$ be the $\alpha$-percentile of $\mu(w(\y, \cdot; \bm{\omega}); \x, \tf, \Lambda, \params)$ in the bootstrap resampling distribution: 
\[Q_{\alpha} \coloneqq \inf_{\mu^*} \left\{\widehat{P}_\D(\mu(w(\y, \cdot; \bm{\omega}); \x, \tf, \Lambda, \params) \leq \mu^*) \geq \alpha \right\}.\]
Finally, let $\params_k$ be the parameters of the model fit on the $k$-th bootstrap sample of the data.
Then, the bootstrap confidence interval of the upper and lower bounds of the CAPO function under the CMSM are given by:
\begin{equation}
    \label{eq:capo_ci}
    \CI_b\left(\mu(\x, \tf; \Lambda, \alpha) \right) \coloneqq \left[ \underline{\mu}_{b}(\x, \tf; \Lambda, \alpha), \overline{\mu}_{b}(\x, \tf; \Lambda, \alpha) \right],
\end{equation}
where,
\begin{equation*}
    \underline{\mu}_{b}(\x, \tf; \Lambda, \alpha) = Q_{\alpha / 2} \left( \left\{ \underline{\mu}(\x, \tf; \Lambda, \params_k)  \right\}_{k = 1}^b \right),
\end{equation*}
and
\begin{equation*}
    \overline{\mu}_{b}(\x, \tf; \Lambda, \alpha) =  Q_{1 - \alpha / 2} \left( \left\{ \overline{\mu}(\x, \tf; \Lambda, \params_k)  \right\}_{k = 1}^b \right).
\end{equation*}
Furthermore, the bootstrap confidence interval of the upper and lower bounds of the APO (dose-response) function under the CMSM are given by:
\begin{equation}
    \label{eq:apo_ci}
    \CI_b\left(\mu(\tf; \Lambda, \alpha) \right) \coloneqq \left[ \underline{\mu}_{b}(\tf; \Lambda, \alpha), \overline{\mu}_{b}(\tf; \Lambda, \alpha) \right],
\end{equation}
where,
\begin{equation*}
    \underline{\mu}_{b}(\tf; \Lambda, \alpha) = Q_{\alpha / 2} \left( \left\{ \underline{\mu}(\tf; \Lambda, \params_k)  \right\}_{k = 1}^b \right),
\end{equation*}
and
\begin{equation*}
    \overline{\mu}_{b}(\tf; \Lambda, \alpha) =  Q_{1 - \alpha / 2} \left( \left\{ \overline{\mu}(\tf; \Lambda, \params_k)  \right\}_{k = 1}^b \right).
\end{equation*}


% \subsubsection{Bayesian interpretation}
% \andrew{Thinking of moving to appendix and leaving for future work}
% Extending the work of \cite{jesson2021quantifying} for binary-valued treatments, we formalize the estimation of $(1 - \alpha)$ credible intervals for the upper and lower bounds under the CMSM.
% \begin{definition}
%     \label{def:bayesion}
%     \normalfont{Monte-Carlo credible interval estimators.}\newline
%     Given, $q(\params \mid \D)$, a variational approximation of the posterior distribution, $p(\params \mid \D)$, over model parameters, $\params$, given the observational data, $\D$. 
%     Sample $k$ times from $q(\params \mid \D)$ to construct a set of functional estimators parameterized by $\{\params_j\}_{j=1}^{k}$.
%     Then, the Monte-Carlo credible interval of the upper and lower bounds of the CAPO function under the CMSM are given by:
%     \begin{equation*}
%         \CrI\left(\mu(\x, \tf), \Lambda, \alpha \right) \coloneqq \left[ \widehat{\underline{\mu}}(\x, \tf; \Lambda, \alpha), \widehat{\overline{\mu}}(\x, \tf; \Lambda, \alpha) \right],
%     \end{equation*}
%     where,
%     \begin{equation*}
%         \widehat{\underline{\mu}}(\x, \tf; \Lambda, \alpha) = Q_{\alpha / 2} \left( \left\{ \widehat{\underline{\mu}}_{\params_j}(\x, \tf; \Lambda)  \right\}_{j = 1}^k \right),
%     \end{equation*}
%     and
%     \begin{equation*}
%         \widehat{\overline{\mu}}(\x, \tf; \Lambda, \alpha) =  Q_{1 - \alpha / 2} \left( \left\{ \widehat{\overline{\mu}}_{\params_j}(\x, \tf; \Lambda)  \right\}_{j = 1}^k \right).
%     \end{equation*}
%     Furthermore, the bootstrap confidence interval of the upper and lower bounds of the APO (dose-response) function under the CMSM are given by:
%     \begin{equation*}
%         \CrI\left(\mu(\tf), \Lambda, \alpha \right) \coloneqq \left[ \widehat{\underline{\mu}}(\tf; \Lambda, \alpha), \widehat{\overline{\mu}}(\tf; \Lambda, \alpha) \right],
%     \end{equation*}
%     where,
%     \begin{equation*}
%         \widehat{\underline{\mu}}(\tf; \Lambda, \alpha) = Q_{\alpha / 2} \left( \left\{ \widehat{\underline{\mu}}_{\params_j}(\tf; \Lambda)  \right\}_{j = 1}^k \right),
%     \end{equation*}
%     and
%     \begin{equation*}
%         \widehat{\overline{\mu}}(\tf; \Lambda, \alpha) =  Q_{1 - \alpha / 2} \left( \left\{ \widehat{\overline{\mu}}_{\params_j}(\tf; \Lambda)  \right\}_{j = 1}^k \right).
%     \end{equation*}
% \end{definition}
